Hardness-Preserving Reductions via Cuckoo Hashing

The focus of this work is \emph{hardness-preserving} transformations of somewhat limited pseudorandom functions families (PRFs) into ones with more versatile characteristics. Consider the problem of \emph{domain extension} of pseudorandom functions: given a PRF that takes as input elements of some domain $U$, we would like to come up with a PRF over a larger domain. Can we do it with little work and without significantly impacting the security of the system? One approach is to first hash the larger domain into the smaller one and then apply the original PRF. Such a reduction, however, is vulnerable to a "birthday attack": after $\sqrt{\size{U}}$ queries to the resulting PRF, a collision (\ie two distinct inputs having the same hash value) is very likely to occur. As a consequence, the resulting PRF is \emph{insecure} against an attacker making this number of queries. In this work we show how to go beyond the aforementioned birthday attack barrier by replacing the above simple hashing approach with a variant of \textit{cuckoo hashing}, a hashing paradigm that resolves collisions in a table by using two hash functions and two tables, cleverly assigning each element to one of the two tables. We use this approach to obtain: (i) a domain extension method that requires {\em just two calls} to the original PRF, can withstand as many queries as the original domain size, and has a distinguishing probability that is exponentially small in the amount of non-cryptographic work; and (ii) a {\em security-preserving} reduction from non-adaptive to adaptive PRFs.

==> PRGImprov.tex <==
\section{Hardness Preserving Construction of PRF from PRG}
In this section we show that using uniform hashing, we can construct PRF from PRG, in such a way that preserve the security of the PRG. This is an improvement to a
construction by \citet{JainPT12}, where they consider a setting where the amount of queries to the the oracle the distinguisher is allowed to ask is strictly less
then is running time. We first describe the setting and construction of \cite{JainPT12}, and then show how to apply uniform hashing to improve it.

\subsection{Hardness Preserving and Good Constructions}
The first construction of PRF from a PRG we introduced by \citet{GoldreichGoMi86}. Bellow we describe their construction.

Let $G\colon \zn \mapsto \zo^{2n}$ be a function, denote by $G_0(s)$ the $\size{s}$-bit long prefix of $G(s)$, and denote by $G_1(s)$ the $\size{s}$-bit long suffix
of $G(s)$. We define $\GGM_G \colon \zn \times \zo^t \mapsto \zn$ to be $\GGM_G(k,x) := G_{x_t}(\cdots (G_{x_2}(G_{x_1}(k))) \cdots)$.

\begin{theorem}[\cite{GoldreichGoMi86}]\label{thm:GGM}
For any $q$-query oracle-aided distinguisher $\Dc$ of running time $T$ there exists a distinguisher $\hcD$ of running time $T+q\cdot t \cdot T_G$ such that
\begin{multline*}
\bsize{\Pr[\hcD(G(U_n)) = 1] - \Pr[\hcD(U_{2n}) = 1]} \geq \frac1{q \cdot t}\cdot\bsize{\Pr_{o \la \GGM_G}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \Pi_n}[\Dc^o(1^n) = 1]},
\end{multline*}
for every $n\in\N$.
\end{theorem}

The construction in \cite{JainPT12}, as do ours, uses $\GGM$ as a black-box. Below we cite two parameters given in \cite{JainPT12}, used to measure a construction
of PRF from PRG.

\begin{definition}[Hardness Preserving Construction]\label{def:HardnessPreserving}
A construction $\F^\ast$ of a PRF from a PRG $G$, is {\sf hardness preserving} up to $q=q(n)$ queries, if for every constants $c>0,\delta>0$ there is a constant
$c'>0$ and $n'\in\N$ such that for all $n>n'$: if $T_G$ is polynomial in $n$ and is $(2^{cn^\delta})$-PRG, then $\F^G$ is $(q,2^{c'n^\delta},2^{-c'n^\delta})$-PRF.
It is hardness preserving if it is hardness preserving for any $q$.

If the above holds for every $c'<c$, we say that it is {\sf strongly} hardness preserving.
\end{definition}

It is conjectured in \cite{JainPT12} that any hardness preserving construction of PRF out of PRG that is secure against $q$ queries must make at least $\Omega(\log
q)$ calls to the PRG per a single invocation of the PRF. This gives the following definition.

\begin{definition}[Good Construction]
A construction as in \cref{def:HardnessPreserving} is {\sf good} for $q$ queries, if it is hardness preserving up to $q$ queries and each call to $\F^G$ results in
$O(\log q)$ calls to $G$. We call is {\sf very good}, if it is even strongly hardness preserving.
\end{definition}

It is shown in \cite{JainPT12} that the known constructions (\ie $\GGM$ and variation of $\GGM$ given by Levin, which in not presented here) are limited when
considering good constructions. They give a new construction, $\JPTCon^G$, depends on a parameter $t$ which denotes the number of calls to $G$ per call to
$\JPTCon^G$, that in some setting, improve known constructions. We will not describe their construction (as it is fairly complicated), but only cite their main
theorem.

\begin{theorem}[\cite{JainPT12}]\label{thm:JPTMain}
If $G$ is $(T',\eps')$-PRG, then $\JPTCon^G$ is $(q,T,\eps)$-PRF, for $T=T'-q\cdot T_{\JPTCon^G} - 3\cdot q \cdot t \cdot n \cdot T_G$, $\eps = 4 \cdot q \cdot t
\cdot \eps' + q^2/2^n + q^t/2^{t^2}$, and every $t,q\in\N$.
\end{theorem}

It is shown in \cite{JainPT12} that when setting $t:=3\log q$, and $q=2^{n^\delta}$, where $0.5 \leq \delta < 1$, then $\JPTCon^G$ is a very good construction.
However, this does not hold for $\delta < 0.5$, \ie $q=2^{o(\sqrt{n})}$. The reason is that the term $q^t/2^{t^2}$ in the size of $\eps$ in \cref{thm:JPTMain} is
not exponentially small when $t = O(\log q)$. Next we give a construction that handle this case as well.

\subsection{Our Construction}
Here we give a simple construction using uniform hashing, that improve \cref{thm:JPTMain}.
\begin{theorem}\label{thm:PRGMain}
Let $\cH= \set{\cH_n \colon \zn \mapsto \zo^t}$ be an efficient $k$-wise independent function family ensemble, let $\cG = \set{\cG_n \colon \zn \mapsto \zn}$ be an
efficient $k$-wise independent function family ensemble, and let $G$ be a $(T'(n),\eps'(n))$-PRG. Then $\PP(\GGM_G)$\footnote{Note that $\cH$ constructing
$\PP(\GGM_G)$ is slightly different than $\PP(\F)$ of \cref{def:PaghPagh}. The reason is that the output length of $\cH$ determine the amount of calls made to $G$,
and we wish to reduce this size to the minimum.} is a $(q,T(n),\eps(n))$-PRF, for $T=T'-p \cdot q\cdot t$, $\eps = 2 \cdot t \cdot q \cdot \eps' + q/2^{c'k}$, large
enough $p\in\poly$ and $4q=2^t$.
\end{theorem}

Before proving \cref{thm:PRGMain}, lets see how it improves \cref{thm:JPTMain}. When setting $k=O(\log^2q)$ we get a result matching \cref{thm:JPTMain}. However, we
have no limitation on setting this value to $k$, and we can improve the security of our construction by increasing it (as long as it is polynomial in $n$). For
example, assume $G$ is $(2^{cn})$-PRG, and we want security against $q=2^{n^{0.4}}$ (which is a case that \cite{JainPT12} do not handle). Setting $k=\log^3q/c'$, we
get that $q/2^{c'k} = 2^{n^{0.4}-n^{1.2}}$, which is smaller than $2^{-cn}$ for large enough $n$. Hence, we get a very good construction. The same argument is
formally put in the following corollary.

\begin{corollary}
For any $c>0$, $0<\delta<1$, $0 < \alpha < \delta$ there exists $k=k(c,\delta,\alpha)$, such that $\PP(\GGM_G)$ is very good for $q=2^{n^\alpha}$ for any $G$ that
is $(2^{cn^\delta})$-PRG.
\end{corollary}
\begin{proof}
Set $k=\lceil\frac{n^\alpha+cn^\delta}{c'}\rceil$. It holds that $\frac{q}{2^{c'k}} < 2^{-cn^\delta}$, and thus $\eps < 2^{1+\log(n^\alpha+2)+n^\alpha-cn^\delta} +
2^{-cn^\delta}$. Let $c''\in\N$ such that $n^{c''} > p(n)$ for large enough $n$, and thus is holds that $T > 2^{cn^\delta} - n^{c''}2^{n^\alpha}(n^\alpha+2)$.
Hence, for every $c'<c$, we have $\eps<2^{-c'n^\delta}$ and $T>2^{c'n^\delta}$ for large enough $n$.
\end{proof}

In order to prove \cref{thm:PRGMain}, we first prove the following lemma.
\begin{lemma}\label{lemma:PRGComputational}
Let $\cH$ ,$\cG$, $G$ and $p$ be as in \cref{thm:PRGMain}. Then for every $q$-query oracle-aided distinguisher $\Dc$ of running time $T$, there exists a
distinguisher $\hcD$ of running time $T(n) + p(n)q(n)\cdot t$, with
\begin{multline*}
\bsize{\Pr[\hcD(G(U_n)) = 1] - \Pr[\hcD(U_{2n}) = 1]} \geq \frac1{2\cdot q \cdot t}\cdot\bsize{\Pr_{o \la \PP(\F)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la
\PP(\Pi)_n}[\Dc^o(1^n) = 1]},
\end{multline*}
for every $n\in \N$.
\end{lemma}
\begin{proof}
Let $\hcD'$ be a two-oracle distinguisher defined as follows:
\begin{algorithm}[$\hcD'$]\label{alg:PRGTwoOracle}
\begin{description}~
\item[Input:] $1^n$.
\item[Oracle:] two functions $\phi_1,\phi_2$ from $\zo^t$ to $\zn$.
\end{description}
\begin{enumerate}
 \item Set $o=\phi_1 \circ h_1 \xor \phi_2 \circ h_2 \xor g$, where $h_1,h_2$ are uniformly chosen in $\cH_n$, and $g$ is uniformly chosen in $\cG_n$.

 \item Emulate $\Dc^o(1^n)$.
\end{enumerate}
\end{algorithm}
Note that $\hcD'$ makes $q$ queries to $\phi_1$ and $\phi_2$, and it can be implemented to run in time $T(n) + q(n)(2T_\cH(n) + T_\cG(n))$. We observe that in case
$\phi_1$ and $\phi_2$ are  uniformly drawn from $\GGM_G$, then the emulation of $\Dc$ done in $\hcD^{\phi_1,\phi_2}$ is identical to a random execution of $\Dc^o$
with $o\la \PP(\GGM_G)_n$. Similarly, in case $\phi_1,\phi_2$ is uniformly drawn from $\Pi_n$, the emulation is identical to a random execution of $\Dc^o$ with
$o\la \PP(\Pi)_n$. Thus,
\begin{multline*}
\bsize{\Pr_{(f_1,f_2) \leftarrow \GGM_G\times\GGM_G}[\hcD'^{f_1,f_2}(1^n) = 1] - \Pr_{(\pi_1,\pi_2) \leftarrow \Pi_n\times\Pi_n}[\hcD'^{\pi_1,\pi_2}(1^n) = 1]}= \\
\bsize{\Pr_{o \la \PP(\GGM_G)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \PP(\Pi)_n}[\Dc^o(1^n) = 1]}.
\end{multline*}
From \cref{lemma:TwoOracle}, we get that there exists a $q$-query single-oracle distinguisher $\hcD''$ of running time $T(n) + q(n)(2T_\cH(n) + T_\cG(n)) +
2T_{\GGM_G}(n)$ such that
\begin{multline*}
\bsize{\Pr_{f \la \GGM_G}[\hcD''^{f}(1^n) = 1] - \Pr_{\pi \la \Pi_n}[\hcD''^{\pi}(1^n) = 1]} \geq \\
\frac12\cdot\bsize{\Pr_{o \la \PP(\GGM_G)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \PP(\Pi)_n}[\Dc^o(1^n) = 1]}.
\end{multline*}
From \cref{thm:GGM} we get that there exists a distinguisher $\hcD$ of running time $T(n) + q(n)(2T_\cH(n) + T_\cG(n)) + 2T_{\GGM_G}(n) + q(n)\cdot t \cdot T_G \leq
T(n) +p(n)q(n)\cdot t$, for large enough $p\in\poly$, such that
\begin{multline*}
\bsize{\Pr[\hcD(G(U_{n})) = 1] - \Pr[\hcD(U_{2n}) = 1]} \geq \\
\frac1{2\cdot q \cdot t}\cdot\bsize{\Pr_{o \la \PP(\GGM_G)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \PP(\Pi)_n}[\Dc^o(1^n) = 1]}.
\end{multline*}
\end{proof}

\cref{thm:PRGMain} follows immediately from the above lemma combine with \cref{lemma:UniStatClose}.


==> PrevSecLoss.tex <==
\section{A Security Preserving Construction}\label{sec:SecPreserving}
\Inote{Start by describing where the security loss is coming from (birthday paradox)}
In this section we improve our basic construction of \cref{sec:construction} by reducing the security loss it induced in \cref{cor:main}, in the cost of a slightly
more complicated construction. This is achieved by using a result by \citet{PaghP08}, where they give a combinatorial construction of a near optimal uniform
hashing. We first describe their result, then define a two-oracle distinguisher needed for the proofs in this section, and lastly apply it to our benefit, using
similar steps to the one we took in \cref{sec:construction}.

\subsection{Uniform Hashing}
The problem of \emph{uniform hashing} is as follows: Given a domain $\cD$ and a range $\cR$, construct a hash function $h\colon \cD \mapsto \cR$ that behaves like a
truly random function from $\cD$ to $\cR$. In order to describe a \emph{truly} random function from $\cD$ to $\cR$ one requires $\Omega(\size{\cD}\log \size{\cR})$ bits. In order to avoid this lower bound, some constructions take a subset $\cT$ of $\cD$ and guarantees that the hash function is uniform over the elements
inside $\cT$. The goal is to construct such restricted hash function, and make it as efficient as possible (where efficiency is measured by the space needed to
present the hash function and the time to evaluate it). \citeauthor{PaghP08}'s main contribution is to describe a restricted uniform hash function that its
efficiency is near optimal. However, even though their main focus and contribution was to achieve the near optimal efficiency, we are only interested in the
analysis of the uniform property of their construction, and not on the efficiency property (as even an optimal function will not be ``efficient'' enough -- it needs
more than a polynomial amount of bits).

Let $T\leq \size{\cD}/4$, let $\cH$ be a function family from $\cD$ to $[4T]_{\cD}$, let $\cG$ be a function family from $\cD$ to $\cR$. For a function family $\cF$
from $\cD$ to $\cR$ define
\begin{align*}
\PP(\cF) = \cF\circ\cH \oplus \cF\circ\cH \oplus \cG.
\end{align*}
\citeauthor{PaghP08}'s construction is $\PP(\Pi)$, where $\Pi$ is the set all functions from $\cD$ to $\cR$ \footnote{Originally, their construction mapped every
$x\in\cD$ to $F_1[h_1(x)]\oplus F_2[h_2(x)] \oplus g(x)$, where $F_1,F_2\in\cR^T$, $h_1,h_2 \colon \cD \mapsto [T]$ that are chosen uniformly from a function family
$\cH$ and $g\colon \cD \mapsto \cR$, that is chosen uniformly from a function family $\cG$. The difference from $\PP(\Pi)$ that we describe above is that we
consider all function from $\cD$ to $\cR$ and not only vectors in $\cR^T$. This only changes the efficiency of the family, that is of no concern to us.}. Their
analysis rests on a bipartite graph $G(h_1,h_1,\cT)$, where $\cT\subseteq\cD$, $h_1,h_1\in\cH$, and on a condition $\Cond(G(h_1,h_1,\cT),k)$ defined over that graph
and an integer $k$. This condition in monotone on $\cT$, namely, for $\cT_1\subseteq\cT_2$ it holds that $\Cond(G(h_1,h_1,\cT_1),k) \Rightarrow
\Cond(G(h_1,h_1,\cT_2),k)$. Since we use their result as a black-box, we will not show how $G(h_1,h_1,\cT)$ is constructed, nor describe the condition itself
(complete details can be found at \cite{PaghP08}). The following lemmas are use to prove the uniform property of $\PP(\Pi)$.

\begin{lemma}\label{lemma:UniNotCond}
Let $\cT\subseteq\cD$ be a set of $T$ elements and let $\cG$ be a function family that is $k$-wise independent on $\cT$. If $\Cond(G(h_1,h_1,\cT),k)$ holds, then
$\PP(\Pi)$ is uniform when restricted to $\cT$.
\end{lemma}

\begin{lemma}\label{lemma:PrCond}
Let $\cT\subseteq\cD$ be of size $T$, and assume that $\cH$ is $k$-wise independent when restricted to $\cT$, then 
$\Pr_{(h_1,h_2) \la \cH^2}[\neg \Cond(G(h_1,h_1,\cT),k)] \leq T/2^{\Omega(k)}$.
\end{lemma}
Set $c'\in\R$ to be a constant such that the probability in \cref{lemma:PrCond} is at most $T/2^{c'k}$.

\subsection{Two Oracle Distinguishers}

\Inote{since this is not an important issue, I would wait with for later}
Before showing how to use the construction of \citeauthor{PaghP08}, we first need to introduce additional framework we use in the proofs of the next section. Note
that a random copy of $\PP(\Pi)$ require two \emph{independent} functions $\pi_1,\pi_2 \la \Pi$. Hence, in order to use similar reduction to the one in
\cref{sec:CompIndist}, we need to define the notion of two oracle distinguisher.

\begin{definition}[psedurandom functions secure against two oracle distinguishers]
An efficient function family ensemble $\F=\set{\F_n\colon \zn \mapsto \zo^{\ell(n)}}_{n \in \N}$ is a {\sf $(T(n),\eps(n))$-two-oracle PRF}, if for every two
oracle-aided algorithm (distinguisher) $\Dc$ of running time $T(n)$ and large enough $n$, it holds that
\begin{align*}
\size{\Pr_{(f_1,f_2) \leftarrow \F_n\times\F_n}[\Dc^{f_1,f_2}(1^n) = 1] - \Pr_{(\pi_1,\pi_2) \leftarrow \Pi_n\times\Pi_n}[\Dc^{\pi_1,\pi_2}(1^n) = 1]} \leq \eps(n),
\end{align*}
where $\Pi_n$ is the set of all functions from $\zn$ to $\zo^{\ell(n)}$. If we limit $\Dc$ above to be non-adaptive, then $\F$ is called {\sf
$(T(n),\eps(n))$-non-adaptive two-oracle PRF}.
\end{definition}

The following lemma is used to link a non-adaptive single oracle PRF to a two oracle one. For a proof of this lemma we refer the reader to \cite{BilletEG10}, where
a more general lemma is proven (the proof in \cite{BilletEG10} does not consider a non-adaptive distinguisher, however it can be easily transfer to this case).

\begin{lemma}[\cf \cite{BilletEG10}, Theorem 1]\label{lemma:TwoOracle}
Assume that $\F = \set{\F_n \colon \zn \mapsto \zo^{\ell(n)}}$ is a function family. Then for every non-adaptive two-oracle distinguisher $\Dc$ of running time
$T(n)$, there exists a non-adaptive single-oracle distinguisher $\hcD$ of running time $p(n)\cdot T(n)$, for some $p\in \poly$ (determined by the computation time
of $\F$), with
\begin{multline*}
\bsize{\Pr_{f \la \F_n}[\hcD^{f}(1^n) = 1] - \Pr_{\pi \la \Pi_n}[\hcD^{\pi}(1^n) = 1]} \geq \\
\frac12\cdot\bsize{\Pr_{(f_1,f_2) \la \F_n\times\F_n}[\Dc^{f_1,f_2}(1^n) = 1]-\Pr_{(\pi_1,\pi_2) \la \Pi_n\times\Pi_n}[\Dc^{\pi_1,\pi_2}(1^n) = 1]},
\end{multline*}
for every $n\in \N$, where $\Pi_n$ is the set of all functions from $\zn$ to $\zo^{\ell(n)}$.
\end{lemma}


\subsection{Applying Uniform Hashing}
In this section we show how to use the above results to improve our basic construction.
\begin{theorem}\label{theorem:UnifomMain}
Let $T$ be a polynomial-time computable integer function, let $\cH= \set{\cH_n \colon \zn \mapsto [4T(n)]_\zn}$ be an efficient $c\log T(n)$ independent function
family ensemble, where $c\in\N$ is a constant to be determined later, let $\cG = \set{\cG_n \colon \zn \mapsto \zn}$ be an efficient $c\log T(n)$ independent
function family ensemble, and let $\F = \set{\F_n \colon \zn \mapsto \zo^{\ell(n)}}$ be a $(p(n)\cdot T(n),\eps(n))$-non-adaptive PRF, where $p \in \poly$ is
determined by the computation time of $T$, $\F$ and $\cH$. Then $\PP(\F)$ is a $(T(n),2\eps(n)+1/T(n))$-adaptive PRF.
\end{theorem}

Again, as in \cref{sec:construction}, \cref{theorem:UnifomMain} yields the following simpler lemma, that reduce the security loss in \cref{cor:main}.

\begin{corollary}\label{cor:UniMain}
Let $T$, $p$, $\cH$ and $\cG$ be as in \cref{theorem:UnifomMain}. Assuming $\F$ is a $\left(p(n)T(n)\right)$-non-adaptive PRF, then $\PP(\F)$ is a
$\left(T(n)/3\right)$-adaptive PRF.
\end{corollary}
\begin{proof}
Applying \cref{theorem:UnifomMain} \wrt $\F$, yields that $\PP(\F)$ is a $\left(T(n),\frac2{p(n)T(n)}+ \frac{1}{T(n)}\right)$-adaptive PRF. Since $\frac2{p(n)T(n)}
\leq \frac2{T(n)}$, it follows that $\PP(\F)$ is a $(T(n)/3,3/T(n))$-adaptive PRF.
\end{proof}

In order to prove \cref{theorem:UnifomMain} we take similar steps to the ones we took to prove \cref{theorem:main}. We use the (non efficient) function family
ensemble $\PP(\Pi)$, where $\Pi = \Pi_\ell$ (\ie the ensemble of all functions from $\zn$ to $\zl$), and $\ell= \ell(n)$ is the output length of $\F$. We first show
that $\PP(\F)$ is \emph{computationally} indistinguishable from $\PP(\Pi)$, and complete the proof showing that $\PP(\Pi)$ is \emph{statistically} indistinguishable
from $\Pi$.

\subsubsection{$\PP(\F)$ is Computationally Indistinguishable From $\PP(\Pi)$}
\begin{lemma}\label{claim:UnifomComClose}
Let $T$, $\F$, $\cH$ and $\cG$ be as in \cref{theorem:UnifomMain}. Then for every oracle-aided distinguisher $\Dc$ of running time $T$, there exists a
\emph{non-adaptive} oracle-aided distinguisher $\hcD$ of running time $p(n)\cdot T(n)$, for some $p\in \poly$ (determined by the computation time of $T$, $\F$,
$\cH$ and $\cG$), with
\begin{multline*}
\bsize{\Pr_{f \la \F_n}[\hcD^{f}(1^n) = 1] - \Pr_{\pi \la \Pi_n}[\hcD^{\pi}(1^n) = 1]} \geq \\
\frac12\cdot\bsize{\Pr_{o \la \PP(\F)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \PP(\Pi)_n}[\Dc^o(1^n) = 1]},
\end{multline*}
for every $n\in \N$, where $\Pi_n$ is the set of all functions from $\zn$ to $\zo^{\ell(n)}$.
\end{lemma}
\begin{proof}
Let $\hcD'$ be a two-oracle distinguisher defined as follows:
\begin{algorithm}[$\hcD'$]\label{alg:UniDis}
\begin{description}~
\item[Input:] $1^n$.
\item[Oracle:] two functions $\phi_1,\phi_2$ over $\zn$.
\end{description}
\begin{enumerate}
 \item \label{Step:UniFirst} Compute $\phi_1(x)$ and $\phi_2(x)$ for every $x \in [4T(n)]_\zn$.

 \item Set $o=\phi_1 \circ h_1 \xor \phi_2 \circ h_2 \xor g$, where $h_1,h_2$ are uniformly chosen in $\cH_n$, and $g$ is uniformly chosen in $\cG_n$.

 \item Emulate $\Dc^o(1^n)$: answer a query $x$ to $\phi_1$ and $\phi_2$ made by $\Dc$ with $o(x)$, using the information obtained in Step \ref{Step:UniFirst}
\end{enumerate}
\end{algorithm}
Note that $\hcD'$ makes \emph{non-adaptive} queries to $\phi_1$ and $\phi_2$, and it can be implemented to run in time $q(n)T(n)$, for large enough $q\in \poly$. We
observe that in case $\phi_1$ and $\phi_2$ are  uniformly drawn from $\F_n$, then the emulation of $\Dc$ done in $\hcD^{\phi_1,\phi_2}$ is identical to a random execution of
$\Dc^o$ with $o\la \PP(\F)_n$. Similarly, in case $\phi_1,\phi_2$ is uniformly drawn from $\Pi_n$, the emulation is identical to a random execution of $\Dc^o$ with
$o\la \PP(\Pi)_n$. Thus,
\begin{multline*}
\bsize{\Pr_{(f_1,f_2) \leftarrow \F_n\times\F_n}[\hcD'^{f_1,f_2}(1^n) = 1] - \Pr_{(\pi_1,\pi_2) \leftarrow \Pi_n\times\Pi_n}[\hcD'^{\pi_1,\pi_2}(1^n) = 1]}= \\
\bsize{\Pr_{o \la \PP(\F)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \PP(\Pi)_n}[\Dc^o(1^n) = 1]}.
\end{multline*}
From \cref{lemma:TwoOracle}, we get that there exists a non-adaptive single-oracle distinguisher $\hcD$ of running time $r(n)q(n)T(n)$, for some $r\in\poly$ such
that
\begin{multline*}
\bsize{\Pr_{f \la \F_n}[\hcD^{f}(1^n) = 1] - \Pr_{\pi \la \Pi_n}[\hcD^{\pi}(1^n) = 1]} \geq \\
\frac12\cdot\bsize{\Pr_{o \la \PP(\F)_n}[\Dc^{o}(1^n) = 1]-\Pr_{o \la \PP(\Pi)_n}[\Dc^o(1^n) = 1]}.
\end{multline*}
We conclude the proof by setting $p = r \cdot q$.
\end{proof}

\subsubsection{$\PP(\Pi)$ is Statistically Indistinguishable From $\Pi$}
\begin{lemma}\label{lemma:UniStatClose}
Let $n,T$ be integers with $T \leq 2^n$, and let $\cH$ and $\cG$ as in \cref{theorem:UnifomMain}. Let $\Dc$ be an (unbounded) $T$-query oracle-aided algorithm (\ie
making at most $T$ queries), then
\begin{align*}
\size{\Pr_{o\la\PP(\Pi)}[\Dc^o = 1] - \Pr_{o\la\Pi}[\Dc^o = 1]} \leq 1/T,
\end{align*}
where $\Pi$ is the set of all functions from $\zn$ to $\zl$ (for some $\ell\in \N$).
\end{lemma}
\begin{proof}
We show that we can apply the general framework presented in \cref{sec:GeneralFramework} to prove this lemma. \Inote{state the lemma here}


In order to show this, we need to define $\cU$, $\cV$,
$\cF$, $\Bad$ and to show that it meets the two properties of \cref{lemma:RandPiClose}. Set $\cU=\cH\times\cH$, $\cV=\Pi\times\Pi\times\cG$, and for
$(h_1,h_2)\in\cU$, $(\pi_1,\pi_2,g)\in\cV$ set $F((h_1,h_1),(\pi_1,\pi_2,g)) = \pi_1\circ h_1 \oplus \pi_2 \circ h_2 \oplus g$. Namely, $\cF(\cU,\cV) = \PP(\Pi)$.
In addition, set $c$ from \cref{theorem:UnifomMain} to be $c=2/c'$ (recall that $c'$ were defined according to \cref{lemma:PrCond}), and set $\Bad =
\set{(\qb,(h_1,h_2))\in (\zn)^{\leq T}\times \cU \colon \neg\Cond(G(h_1,h_2,\qb),c\log T)}$.

\cref{lemma:UniNotCond} assures that property $1$ of \cref{lemma:RandPiClose} is satisfied, and according to \cref{lemma:PrCond} we set $\eps$ of
\cref{lemma:RandPiClose} to be $T/2^{c'c\log T} = 1/T$, and thus property $2$ is also satisfied. Finally, setting $s=T$, the proof follows immediately from
\cref{lemma:RandPiClose}.
\end{proof}

\subsubsection{Putting It Together}
We are now finally ready to prove \cref{theorem:UnifomMain}.
\begin{proof}[Proof of \cref{theorem:UnifomMain}]
Let $\Dc$ be an oracle-aided algorithm of running time $T(n)$. \cref{claim:UnifomComClose} yields that $\size{\Pr_{o \la \PP(\F)}[\Dc^{o}(1^n) = 1] - \Pr_{o \la
\PP(\Pi)}[\Dc^{o}(1^n) = 1]} \leq 2\eps(n)$ for large enough $n$, where \cref{lemma:UniStatClose} yields that $\size{\Pr_{o \la \PP(\Pi)}[\Dc^{o}(1^n) = 1] -
\Pr_{\pi \la \Pi_n}[\Dc^{\pi}(1^n) = 1]} \leq 1/T(n)$ for every $n\in \N$. Hence, the triangle inequality yields that $\size{\Pr_{o \la \PP(\F)}[\Dc^{o}(1^n) = 1] -
\Pr_{\pi \la \Pi_n}[\Dc^{\pi}(1^n) = 1]} \leq 2\eps(n) + 1/T(n)$ for large enough $n$, as requested.
\end{proof}

